Towards more efficient quantitative safety validation of residual risk for assisted and automated driving

The safety validation of Advanced Driver Assistance Systems (ADAS) and Automated Driving Systems (ADS) increasingly demands efficient and reliable methods to quantify residual risk while adhering to international standards such as ISO 21448. Traditionally, Field Operational Testing (FOT) has been pivotal for macroscopic safety validation of automotive driving functions up to SAE automation level 2. However, state-of-the-art derivations for empirical safety demonstrations using FOT often result in impractical testing efforts, particularly at higher automation levels. Even at lower automation levels, this limitation - coupled with the substantial costs associated with FOT - motivates the exploration of approaches to enhance the efficiency of FOT-based macroscopic safety validation. Therefore, this publication systematically identifies and evaluates state-of-the-art Reduction Approaches (RAs) for FOT, including novel methods reported in the literature. Based on an analysis of ISO 21448, two models are derived: a generic model capturing the argumentation components of the standard, and a base model, exemplarily applied to Automatic Emergency Braking (AEB) systems, establishing a baseline for the real-world driving requirement for a Quantitative Safety Validation of Residual Risk (QSVRR). Subsequently, the RAs are assessed using four criteria: quantifiability, threats to validity, missing links, and black box compatibility, highlighting potential benefits, inherent limitations, and identifying key areas for further research. Our evaluation reveals that, while several approaches offer potential, none are free from missing links or other substantial shortcomings. Moreover, no identified alternative can fully replace FOT, reflecting its crucial role in the safety validation of ADAS and ADS.

==> setup/new_commands.tex <==
\makeatletter
\newcommand{\AH}{$A_{\mathrm{H}}$}
\newcommand{\taui}{$\tau_{\mathrm{i}}$}
\newcommand{\VTi}{$\mathrm{VTs}$}%
\newcommand{\validationtarget}{\gls{VT}}
\newcommand{\validationtargets}{\glspl{VT}}
\newcommand{\BaseModel}{Base Model}
\newcommand{\basemodel}{\textit{base model}}
\newcommand{\GenericModel}{Generic Model}
\newcommand{\genericmodel}{\textit{generic model}}
\newcommand{\FigApproachPrefix}{Reduction Approach: }
\newcommand{\macroscopicrisk}{\textit{macroscopic risk}}
\newcommand{\residualrisk}{\textit{residual risk}}

\newcommand{\DefineCriterion}[3]{%
  \expandafter\newcommand\csname #1Name\endcsname{#2}%
  \expandafter\newcommand\csname #1name\endcsname{\MakeLowercase{\csname #1Name\endcsname}}%
 \expandafter\newcommand\csname #1\endcsname[1][]{\hyperref[sec::#1]{\ifstrempty{##1}{\textit{\csname #1name\endcsname}}{\textit{##1}}}}%
  \expandafter\newcommand\csname #1ShortName\endcsname{#3}%
  \expandafter\newcommand\csname #1Shortname\endcsname{\MakeLowercase{\csname #1ShortName\endcsname}}%
  \expandafter\newcommand\csname #1Short\endcsname{\hyperref[sec::#1]{\textit{\csname #1ShortName\endcsname}}}%
  \expandafter\newcommand\csname #1short\endcsname{\hyperref[sec::#1]{\textit{\csname #1Shortname\endcsname}}}%
}
\DefineCriterion{CritQuantifiablity}{Quantifiability of the Effect}{Quantifiability}
\DefineCriterion{CritValidity}{Threats to Validity}{Threats to Validity}
\DefineCriterion{CritMissingLinks}{Missing Links for Application}{Missing Links}
\DefineCriterion{CritBlackbox}{Black-Box Compatibility}{Black-Box Comp.}

\newcommand\Positive{$\oplus$}
\newcommand\Negative{$\ominus$}
\newcommand\Neutral{$\circledcirc$}

\newcommand{\RCReevaluation}{Reevaluation of Assumptions, Requirements, and Inference}
\newcommand{\RCUncertainty}{Reduction of Uncertainty or Variance}
\newcommand{\RCSupplement}{Supplementation or Substitution of FOT data}

\newcommand{\RPEquivalentCriteria}{Derivation of Equivalent Acceptance Criteria}
\newcommand{\RPLoweringRequirements}{Lowering of the Certainty Requirements}
\newcommand{\RPAlternativeInference}{Utilization of Alternative Statistical Inference}
\newcommand{\RPExpertKnowledge}{Expert Knowledge with Similar Systems}
\newcommand{\RPTestProfile}{Test Profile Refinement}
\newcommand{\RPValueEstimation}{Estimation Improvement}
\newcommand{\RPSimBT}{Simulation-based Testing}
\newcommand{\RPPGT}{Proving Ground Testing}

\newcommand{\RADecompositionAH}{Decomposition of Acceptance Criterion}
\newcommand{\RADecompositionHB}{Decomposition of Hazardous Behavior}
\newcommand{\RARedundancy}{Redundancy and Independence Considerations}
\newcommand{\RASequentialTesting}{Sequential Testing}
\newcommand{\RABayesianStatistics}{Bayesian Statistics}
\newcommand{\RAHighYieldRouteProfiles}{High Yield Route Profiles}
\newcommand{\RAEVA}{Extreme Value Analysis}
\newcommand{\RAVirtualFOT}{Virtual FOT}
\newcommand{\RASBT}{Scenario Based Testing}

\newcommand{\figureref}[1]{Fig.~\ref{#1}}
\newcommand{\tableref}[1]{Table~\ref{#1}}
\newcommand{\sectionref}[1]{Section~\ref{#1}}
\newcommand{\subsectionref}[1]{Subsection~\ref{#1}}
\newcommand{\paragraphref}[1]{Paragraph~\ref{#1}}
\newcommand{\equationref}[1]{(\ref{#1})}
\newcommand{\we}{we}
\newcommand{\We}{We}
\newcounter{RP}
\newcounter{RC}
\newcounter{RA}
\newcommand{\RCSubSection}[1]{\refstepcounter{RC}\subsection*{\hyperref[fig::Reduction_Path_overview]{RC: #1}}}
\newcommand{\RPSubSubSection}[1]{\refstepcounter{RP}\subsubsection*{\hyperref[fig::Reduction_Path_overview]{RP: #1}}}
\newcommand{\RAParagraph}[1]{\refstepcounter{RA}\paragraph*{\hyperref[fig::Reduction_Path_overview]{RA: #1}}}

\newcounter{SOTIFClauseNumber}
\setcounter{SOTIFClauseNumber}{4}
\newcounter{GenericModelNumber}
\newcounter{BaseModelNumber}


\newcommand{\subsubsectionWithLink}[2]{%
    \subsubsection{\texorpdfstring{\hyperref[#1]{#2}}{#2}}%
}
\makeatother

\input{setup/setup_tikz}
\input{setup/tikz_commands_for_generic_model}

\makeatletter
\newcommand{\SotifClause}[2][scale=0.8]{%
  \tikzexternaldisable\begin{tikzpicture}[baseline={([yshift=-1pt]C#2.base)}]
    \node[number, inner sep = 0pt, minimum size=.42cm,#1](C#2) {\hyperref[fig::SOTIF_overview]{\textbf{#2}}};
  \end{tikzpicture}\tikzexternalenable%
}
\newcommand{\SotifClauseref}[2][scale=0.8]{%
\sectionref{sec::SOTIFSummary}~%
  \tikzexternaldisable\begin{tikzpicture}[baseline={([yshift=-1pt]C.base)}]
    \node[number, inner sep = 0pt, minimum size=.42cm,#1](C) {\hyperref[#2]{\textbf{\ref{#2}}}};
  \end{tikzpicture}\tikzexternalenable%
}

\newcommand{\ComponentGenericModel}[2][scale=0.8]{%
\tikzexternaldisable\begin{tikzpicture}[baseline={([yshift=-1pt]G#2.base)}]
    \node[number, minimum size=.42cm,#1, generic, fill=white, text= black, draw=black](G#2) {\hyperref[fig::Generic_Model]{\textbf{#2}}};
\end{tikzpicture}\tikzexternalenable%
}

\newcommand{\GenericModelref}[2][scale=0.8]{%
\sectionref{sec::generic_model}~%
\tikzexternaldisable\begin{tikzpicture}[baseline={([yshift=-1pt]G.base)}]
    \node[number, minimum size=.42cm,#1, generic, fill=white, text= black, draw=black](G) {\hyperref[#2]{\textbf{\ref{#2}}}};
\end{tikzpicture}\tikzexternalenable%
}

\newcommand{\BaseModelComponent}[2][scale=0.8]{%
\tikzexternaldisable\begin{tikzpicture}[baseline={([yshift=-1pt]B#2.base)}]
    \node[number, minimum size=.42cm,#1, implemented, text= black, draw=black](B#2) {\hyperref[fig::Base_Model]{\textbf{#2}}};
\end{tikzpicture}\tikzexternalenable%
}
\newcommand{\BaseModelref}[2][scale=0.8]{%
\sectionref{sec::base-model}~%
\tikzexternaldisable\begin{tikzpicture}[baseline={([yshift=-1pt]B.base)}]
    \node[number, minimum size=.42cm,#1, implemented, text= black, draw=black](B) {\hyperref[#2]{\textbf{\ref{#2}}}};
\end{tikzpicture}\tikzexternalenable%
}

\NewDocumentCommand{\subsubsectionClause}{m o }{%
\refstepcounter{SOTIFClauseNumber}%
\subsubsection*{%
\texorpdfstring{%
\SotifClause{\theSOTIFClauseNumber}~\hyperref[fig::SOTIF_overview]{#1}%
}{%
\IfNoValueTF{#2}{%
\theSOTIFClauseNumber #1%
}{%
\theSOTIFClauseNumber{}#2%
}%
}%
}%
}

\NewDocumentCommand{\subsubsectionGenericModel}{m o }{%
\refstepcounter{GenericModelNumber}%
\subsubsection*{%
\texorpdfstring{%
\ComponentGenericModel{\theGenericModelNumber}~\hyperref[fig::Generic_Model]{#1}%
}{%
\IfNoValueTF{#2}{%
\theGenericModelNumber #1%
}{%
\theGenericModelNumber #2%
}%
}%
}%
}

\NewDocumentCommand{\subsubsectionBaseModel}{ m o }{%
\refstepcounter{BaseModelNumber}%
\subsubsection*{%
\texorpdfstring{%
\BaseModelComponent{\theBaseModelNumber}~\hyperref[fig::Base_Model]{#1}%
}{%
\IfNoValueTF{#2}{%
\theBaseModelNumber #1%
}{%
\theBaseModelNumber #2%
}%
}%
}%
}

\makeatother

\makeatletter
\newcommand*{\getbeforecolon}[1]{%
  \begingroup
    \edef\bbx@temp{#1:}%
    \expandafter\get@beforecolon\bbx@temp\relax
  \endgroup
}
\def\get@beforecolon#1:#2\relax{#1}
\makeatother

\DeclareCiteCommand{\citenum}
  {\begingroup}
  {\edef\bbx@temp{\thefield{number}}%
  \getbeforecolon{\bbx@temp}%
  }{}{\endgroup}
\newcommand{\citenumber}[1]{\begingroup\boolfalse{citerequest}\citenum{#1}\endgroup}


==> setup/setup_tikz.tex <==

\usetikzlibrary{
  arrows,
  arrows.meta,
  calc,
  fit,     
  intersections,
  math,
  matrix,
  positioning,
  shapes,
  trees
}

\tikzstyle{block}     = [draw, rectangle, minimum height=6mm, minimum width=8mm, inner sep=1mm, text width = 1cm]
\tikzstyle{blockText} = [draw, rectangle, minimum height = 6 mm, minimum width=8mm, inner sep=1 pt, align=center,text width=20mm]
\tikzstyle{number} =[circle, fill=black, text=white, circle, font=\footnotesize, text centered, inner sep =0.5pt, minimum size=0.35cm]
\tikzset{every picture/.style={font=\footnotesize}}

\tikzset{
  hyperref node/.style={
    alias=sourcenode,
    append after command={%
      \bgroup
        [current point is local=true]
        let \n0={\pgfkeysvalueof{/pgf/outer xsep}},
            \n1={\pgfkeysvalueof{/pgf/outer ysep}},
            \p1= (sourcenode.south west),
            \p2= (sourcenode.north east),
            \n2={\x2-\x1},
            \n3={\y2-\y1} 
        in
        node[
          at=(\p1),
          draw=none,
          shape=rectangle,
          inner sep=0pt,
          outer sep=0pt,
          minimum width=0pt,
          minimum height=0pt,
        ]{%
          \rlap{%
            \raisebox{0pt}[0pt][0pt]{%
              \hyperref[#1]{%
                \phantom{\rule{\n2}{\n3}}%
              }%
            }%
          }%
        }%
      \egroup
    },
  }
}

\tikzset{
  hyperref circle/.style={
    alias=sourcenode,
    append after command={%
      \bgroup
        [current point is local=true]
        let \n0={\pgfkeysvalueof{/pgf/outer xsep}},
            \n1={\pgfkeysvalueof{/pgf/outer ysep}},
            \p1= (sourcenode.south west),
            \p2= (sourcenode.north east),
            \n2={\x2-\x1},
            \n3={\y2-\y1} 
        in
        node[
          at=(\p1),
          draw=none,
          shape=circle,
          inner sep=0pt,
          outer sep=0pt,
          minimum width=0pt,
          minimum height=0pt,
        ]{%
          \rlap{%
            \raisebox{0pt}[0pt][0pt]{%
              \hypertarget{link::{#1}Picture}{\hyperref[#1]{%
                \phantom{\rule{\n2}{\n3}}%
              }}%
            }%
          }%
        }%
      \egroup
    },
  }
}



\tikzset{
  hyperlink node/.style={
    alias=sourcenode,
    append after command={%
      \bgroup
        [current point is local=true]
        let \n0={\pgfkeysvalueof{/pgf/outer xsep}},
            \n1={\pgfkeysvalueof{/pgf/outer ysep}},
            \p1= (sourcenode.south west),
            \p2= (sourcenode.north east),
            \n2={\x2-\x1},
            \n3={\y2-\y1} 
        in
        node[
          at=(\p1),
          draw=none,
          shape=rectangle,
          inner sep=0pt,
          outer sep=0pt,
          minimum width=0pt,
          minimum height=0pt,
        ]{%
          \rlap{%
            \raisebox{0pt}[0pt][0pt]{%
              \hypertarget{link::#1Picture}{\hyperlink{link::#1Text}{%
                \phantom{\rule{\n2}{\n3}}%
              }%
              }%
            }%
          }%
        }%
      \egroup
    },
  }
}


==> setup/tikz_commands_for_generic_model.tex <==

\makeatletter

\tikzset{
    legend/.style={
      draw,
      above left,
      row sep=2pt ,
      column sep=2 pt,
      inner sep=1.5pt
    },
    connector/.style={
      -{Latex[length=1mm, width=1mm]},
      shorten >=0.02pt,
      shorten <=0.02,
      rounded corners=1pt
    },
    componentinput/.style={
      draw,
      fill=white,
      rectangle,
      inner sep=0.7pt,
      outer sep=0pt,
      anchor = east,
      font=\tiny
    },
    componentoutput/.style={
      draw,
      fill=white,
      rectangle,
      inner sep=0.7pt,
      outer sep=0pt,
      anchor = west,
      font=\tiny
    },
    input_old/.style={
      draw,
      circle,
      minimum size=1.8 cm,
      font=\footnotesize,
      text width= 1.6 cm,
      inner sep=-2pt,
      text centered,
      anchor = north
    },
    input/.style={
      draw,
      signal,
      font=\footnotesize,
      inner sep=2 pt,
      align = center,
      text centered,
      anchor = north east
    },
  component/.style args={inputs #1 and outputs #2}{
    draw,
    minimum width=1.9cm,
    minimum height=1cm,
    font=\footnotesize,
    align = center,
    inner sep=2 pt,
    rounded corners=2pt,
    text centered,
    anchor = west,
    append after command={
      \pgfextra{
        \StrLen{#1}[\numinputslen]
        \StrLen{#2}[\numoutputslen]
        \StrCount{#1}{x}[\numinputs]
        \StrCount{#2}{x}[\numoutputs]
        \ifnum\numinputs>0
          \newcount\numbinputs
          \numbinputs=0
          \foreach \x in {1,...,\numinputslen} {
            \StrChar{#1}{\x}[\char]
            \IfStrEq{\char}{x}{%
              \global\advance\numbinputs by 1
              \node [componentinput] (\tikzlastnode-input\the\numbinputs) at ($(\tikzlastnode.north west)!{\x/(\numinputslen+1)}!(\tikzlastnode.south west)$) {};
            }
          }
        \fi
        \ifnum\numoutputs>0
          \newcount\numboutputs
          \numboutputs=0
          \foreach \x in {1,...,\numoutputslen} {
            \StrChar{#2}{\x}[\char]
            \IfStrEq{\char}{x}{
              \global\advance\numboutputs by 1
              \node [componentoutput] (\tikzlastnode-output\the\numboutputs) at ($(\tikzlastnode.north east)!{\x/(\numoutputslen+1)}!(\tikzlastnode.south east)$) {};
            }
          }
        \fi
      }
    },
  },
  generic/.style={
      fill=gray!10,
    },
  implemented/.style={
      fill=DarkBlue!10,
    },
  additional/.style={
      fill=DarkGreen!10,
    },
  additionalLine/.style={
      color = Green!50!black,
      text=Green!50!black
    },
  implementedLine/.style={
      color = DarkBlue!50!black,
      text= DarkBlue!50!black
    },
  genericLine/.style={
      color = black,
      text=black
    },
  newLine/.style={
      color = red!50!black,
      text=red!50!black
    },
  new/.style={
    fill = red!20!white,
    draw = red!50!black,
    text=red!50!black
  },
  clabel/.style={
      fill=white,
      scale=0.8,
      inner sep= 0.5pt, 
      align = center, 
      anchor = center
    },
  newClabel/.style={
      text=red!50!black,
      clabel
    },
  genericCLabel/.style={
      text=black,
      clabel
    },
  implementedCLabel/.style={
      text=DarkBlue!50!black,
      clabel
    },
  additionalCLabel/.style={
      text=Green!50!black,
      clabel
    }
}
\makeatother

\newcommand{\PlaceNewLabel}[6][]{%
    \coordinate (start) at (#2.east);
    \coordinate (end) at (#3.west);
    \coordinate (hRef) at ($(start)!#4!(end)$);
    \coordinate (vRef) at ($(start)!#5!(end)$);
    \ifx#1\empty
        \node[clabel, text = red!50!black] at (hRef|-vRef) {#6};
    \else
      \node[clabel, text = red!50!black,#1] at (hRef|-vRef) {#6};
    \fi
}
\tikzstyle{multiline}		=	[solid]
\tikzset{
  avoid intersection amplitude/.store in=\avint@amplitude,
  avoid intersection width/.code={\edef\avint@width{\dimexpr#1/2}},
  avoid intersection offset/.store in=\avint@offset,
  avoid intersection has corners/.code={\pgfdecoratepathhascornerstrue}
}
\def\avint@amplitude{5pt}
\def\avint@width{5pt}
\def\avint@offset{0pt}

\pgfdeclaredecoration{avoidintersect}{initial}{
  \state{initial}[width=\pgfdecoratedinputsegmentlength/100,next state=measure]
  {
    \gdef\avint@intersectionnumber{1}
    \pgfpathlineto{\pgfpointorigin}
  }

  \state{measure}[width=\pgfdecoratedinputsegmentlength/100,next state=wait,auto corner on length=2pt,
               persistent postcomputation=\let\pgf@decorate@next@state\avint@smuggle@pgf@decorate@next@state]
  {
    \pgfpathlineto{\pgfpointorigin}
    \pgfgettransform\avint@temptransform
    \pgftransforminvert
    \pgfpointintersectionsolution{\avint@intersectionnumber}
    \pgf@pos@transform{\pgf@x}{\pgf@y}
    \pgfmathveclen{\pgf@x}{\pgf@y}
    \pgfsettransform\avint@temptransform
    \xdef\avint@waitcycles{\the\numexpr\dimexpr\pgfmathresult pt-\avint@width*3-\avint@offset\relax/\dimexpr\pgfdecoratedinputsegmentlength/100\relax}
    \ifnum\avint@waitcycles>50\relax\gdef\avint@waitcycles{50}\fi
    \global\let\avint@smuggle@pgf@decorate@next@state\pgf@decorate@next@state        
    \ifdim\pgfmathresult pt<\dimexpr\avint@width+\avint@offset\relax
        \gdef\avint@smuggle@pgf@decorate@next@state{zig}
    \else
        \ifdim\pgfmathresult pt<\dimexpr\avint@width*2+\avint@offset\relax
            \gdef\avint@smuggle@pgf@decorate@next@state{measure}    
        \fi
    \fi        
  }

  \state{wait}[width=\pgfdecoratedinputsegmentlength/100,next state=measure,repeat state=\avint@waitcycles,auto corner on length=2pt]{
    \pgfpathlineto{\pgfpointorigin}
  } 

  \state{zig}[width=\avint@width, next state=zag]{
    \pgfpathcurveto{\pgfqpoint{\avint@width}{0cm}}{\pgfqpoint{0pt}{\avint@amplitude}}{\pgfqpoint{\avint@width}{\avint@amplitude}}
  }
  \state{zag}[width=\avint@width, next state=measure,
              persistent postcomputation=\let\pgf@decorate@next@state\avint@smuggle@pgf@decorate@next@state]{
    \pgfpathcurveto{\pgfqpoint{\avint@width}{\avint@amplitude}}{\pgfqpoint{0pt}{0cm}}{\pgfqpoint{\avint@width}{0pt}}
    \xdef\avint@intersectionnumber{\the\numexpr\avint@intersectionnumber+1}
    \global\let\avint@smuggle@pgf@decorate@next@state\pgf@decorate@next@state
    \ifnum\avint@intersectionnumber>\pgfintersectionsolutions
      \gdef\avint@smuggle@pgf@decorate@next@state{done}
    \fi
  }

  \state{done}[width=\pgfdecoratedinputsegmentlength/100,auto corner on length=2pt]{
    \pgfpathlineto{\pgfpointorigin}
  }

  \state{final}{\pgfpathlineto{\pgfpointdecoratedpathlast}}
}    

\tikzset{
    avoid intersection/.code 2 args={
        \pgfkeysalso{name path=avint@temp,draw=none}
        \expandafter\def\expandafter\tikz@postactions\expandafter{\tikz@postactions
            \pgfintersectionsortbyfirstpath
            \tikz@intersect@namedpaths
            \pgfintersectionofpaths
                {\pgfsetpath\tikz@intersect@path@name@avint@temp}
                {\expandafter\pgfsetpath\csname tikz@intersect@path@name@#1\endcsname}
            \begin{pgfdecoration}{{avoidintersect}{\pgfdecoratedpathlength}}
            \pgfsetpath\tikz@intersect@path@name@avint@temp
            \end{pgfdecoration}
            \pgfgetpath\avint@temp@path
            \pgfusepath{discard}
            \draw[/utils/exec={\tikz@addmode{\pgfsyssoftpath@setcurrentpath\avint@temp@path}},#2](0,0)rectangle (0,0);%
        }
    }
}
\makeatother
\makeatletter

\long\def\ifnodedefinedglobal#1#2{%
    \@ifundefined{pgf@sh@ns@#1}{}{#2}%
}
\makeatother
\makeatletter
\newcommand{\hideFlag}[2]{%
  \ifcsname #1\endcsname
  \else
    #2
  \fi
}
\makeatother
\makeatletter
\long\def\ifnodedefined#1#2{%
   \expandafter\ifx\csname pgf@sh@pi@#1\endcsname\pgfpictureid
      #2
   \fi
}
\makeatother
\makeatletter
\newcommand{\tikzifdefined}[3]{%
   \ifcsname #1\endcsname
      #2
    \else
      #3
   \fi
}
\newcommand{\Line}[1]{#1Line}
\newcommand{\CLabel}[1]{#1CLabel}
\makeatother
\definecolor{DarkBlue}{rgb}{0,0,.545}
\definecolor{DarkGreen}{rgb}{0,.392,0}
\definecolor{Green}{rgb}{0,0.75,0}

